M$^2$-Miner: Multi-Agent Enhanced MCTS for Mobile GUI Agent Data Mining

Graphical User Interface (GUI) agent is pivotal to advancing intelligent human-computer interaction paradigms. Constructing powerful GUI agents necessitates the large-scale annotation of high-quality user-behavior trajectory data (i.e., intent-trajectory pairs) for training. However, manual annotation methods and current GUI agent data mining approaches typically face three critical challenges: high construction cost, poor data quality, and low data richness. To address these issues, we propose M$^2$-Miner, the first low-cost and automated mobile GUI agent data-mining framework based on Monte Carlo Tree Search (MCTS). For better data mining efficiency and quality, we present a collaborative multi-agent framework, comprising InferAgent, OrchestraAgent, and JudgeAgent for guidance, acceleration, and evaluation. To further enhance the efficiency of mining and enrich intent diversity, we design an intent recycling strategy to extract extra valuable interaction trajectories. Additionally, a progressive model-in-the-loop training strategy is introduced to improve the success rate of data mining. Extensive experiments have demonstrated that the GUI agent fine-tuned using our mined data achieves state-of-the-art performance on several commonly used mobile GUI benchmarks. Our work will be released to facilitate the community research.

==> Sections/3_preliminary.tex <==
\section{Preliminary: Monte Carlo Tree Search}
Monte Carlo Tree Search is a heuristic tree search algorithm widely used in sequential decision-making tasks. Unlike traditional tree search methods that rely on handcrafted evaluation functions, MCTS dynamically constructs a search tree through iterative simulations, balancing exploration and exploitation using statistical estimates. Each node in the tree represents a state in the environment, and each edge corresponds to an action that transitions the environment to a new state.

At the core of MCTS lies a four-step procedure repeated at each iteration: \textit{Selection}, \textit{Expansion}, \textit{Simulation}, and \textit{Backpropagation}. 
% 具体来说
Specifically, during the selection phase, the algorithm traverses the search tree and selects a node using a principled selection policy. 
A commonly used policy is the Upper Confidence Bounds applied to Trees (UCT)~\cite{mcts_kocsis2006bandit}, which balances exploitation and exploration by choosing actions that maximize:
\begin{equation}
    a^* = \arg\max_{a\in\mathcal{A}(s)} \left\{ \bar{Q}(s,a) + c \sqrt{\frac{\ln N(s)}{N(s,a)}} \right\},
\end{equation}
where $\bar{Q}(s,a)$ is the cumulative reward of the child node that is obtained by taking action $a$ in state $s$, $N(s)$ represents the visit count for state $s$, $N(s,a)$ denotes the number of times action $a$ has been taken in state $s$, and $c>0$ is a constant controlling the exploration-exploitation trade-off. After a node is selected, an action is randomly chosen in the expansion phase to obtain a child node. Subsequently, in the simulation phase, the algorithm conducts a complete process (roll-out) starting from this newly expanded node until a terminal state is reached. 
This process typically follows a simple and fast policy, such as making decisions completely at random. 
The purpose of the roll-out is to quickly obtain a result or evaluation, such as a reward. 
The backpropagation phase begins after the rollout concludes and a reward is obtained. During this phase, the algorithm backtracks from the newly expanded node up to the root, utilizing the simulation results to update the statistical information of all nodes along the path, such as their visit counts and cumulative rewards (\textit{e.g.}, number of successes).

Despite its effectiveness, vanilla MCTS suffers from computational inefficiency in large or complex environments (\textit{e.g.}, GUI agent task). Specifically, because vanilla MCTS randomly selects actions for expansion and relies on repeated rollouts to obtain rewards, its applicability is restricted in high-dimensional or real-time applications.
